Shifting AI Efficiency From Model-Centric to Data-Centric Compression

The advancement of large language models (LLMs) and multi-modal LLMs (MLLMs) has historically relied on scaling model parameters. However, as hardware limits constrain further model growth, the primary computational bottleneck has shifted to the quadratic cost of self-attention over increasingly long sequences by ultra-long text contexts, high-resolution images, and extended videos. In this position paper, \textbf{we argue that the focus of research for efficient artificial intelligence (AI) is shifting from model-centric compression to data-centric compression}. We position data-centric compression as the emerging paradigm, which improves AI efficiency by directly compressing the volume of data processed during model training or inference. To formalize this shift, we establish a unified framework for existing efficiency strategies and demonstrate why it constitutes a crucial paradigm change for long-context AI. We then systematically review the landscape of data-centric compression methods, analyzing their benefits across diverse scenarios. Finally, we outline key challenges and promising future research directions. Our work aims to provide a novel perspective on AI efficiency, synthesize existing efforts, and catalyze innovation to address the challenges posed by ever-increasing context lengths.

==> tables/Mistral_series.tex <==
\begin{table*}[t!]
\centering
\caption{\textbf{Mistral series model specifications.} Includes release timelines, parameter scales, and context capabilities.}
\vspace{2mm}
{\fontsize{9}{11}\selectfont
\renewcommand{\arraystretch}{1.0}
\setlength\tabcolsep{11pt}
\begin{tabular}{lcccc}
\textbf{Model Name} & \textbf{Release Date} & \textbf{Parameters} & \textbf{Context Length} & \textbf{Model Link} \\
\shline
Mistral-7B          & Sep 2023    & 7B                 & 8K (SW)                 & \href{https://huggingface.co/mistralai/Mistral-7B-v0.1}{link} \\
Mistral-7B          & Feb 2024              & 7B                 & 8K (SW)                 & \href{https://huggingface.co/mistralai/Mistral-7B-v0.2}{link} \\
Mistral-7B          & Early 2024            & 7B                 & 8K (SW)                 & \href{https://huggingface.co/mistralai/Mistral-7B}{link} \\
\hline
Mixtral-8x7B        & Dec 2023              & 45B (12.9B active) & 32K                     & \href{https://huggingface.co/mistralai/Mixtral-8x7B}{link} \\
Mixtral-8x22B       & Apr 2024              & 141B (39B active)  & 64K                     & \href{https://huggingface.co/mistralai/Mixtral-8x22B}{link} \\
\hline
Mistral Nemo        & Jul 2024              & 12B                & 128K                    & \href{https://huggingface.co/mistralai/Mistral-Nemo}{link} \\
Mistral Large       & Feb 2024              & Not disclosed      & 32K                     & \href{https://huggingface.co/mistralai/Mistral-Large}{link} \\
Mistral Large 2     & Jul 2024              & 123B               & 128K                    & \href{https://huggingface.co/mistralai/Mistral-Large-2}{link} \\
Mistral Large 2     & Nov 2024              & 123B               & 128K                    & \href{https://huggingface.co/mistralai/Mistral-Large-2-v2}{link} \\
\hline
Ministral 3B        & Oct 2024              & 3B                 & 128K$^\ddagger$         & \href{https://huggingface.co/mistralai/Ministral-3B}{link} \\
Ministral 8B        & Oct 2024              & 8B                 & 128K$^\ddagger$         & \href{https://huggingface.co/mistralai/Ministral-8B}{link} \\
\hline
Mistral Small       & Feb 2024              & Not disclosed      & 32K                     & \href{https://huggingface.co/mistralai/Mistral-Small-v1}{link} \\
Mistral Small       & Sep 2024              & Not disclosed      & 32K                     & \href{https://huggingface.co/mistralai/Mistral-Small-v2}{link} \\
Mistral Small 3     & Jan 2025              & 24B                & 32K                     & \href{https://huggingface.co/mistralai/Mistral-Small-3}{link} \\
\rowcolor[rgb]{ .949,  .949,  .949}
Mistral Small 3.1   & Mar 2025              & 24B                & 128K                    & \href{https://huggingface.co/mistralai/Mistral-Small-3.1}{link} \\
Mistral Medium 3    & May 2025              & Not disclosed      & 130K                    & \href{https://huggingface.co/mistralai/Mistral-Medium-3}{link} \\
\end{tabular}
}
\label{tab:mistral_specs}
\end{table*}

